On Monotonic Aggregation for Open-domain QA

Question answering (QA) is a critical task for speech-based retrieval from knowledge sources, by sifting only the answers without requiring to read supporting documents. Specifically, open-domain QA aims to answer user questions on unrestricted knowledge sources. Ideally, adding a source should not decrease the accuracy, but we find this property (denoted as "monotonicity") does not hold for current state-of-the-art methods. We identify the cause, and based on that we propose Judge-Specialist framework. Our framework consists of (1) specialist retrievers/readers to cover individual sources, and (2) judge, a dedicated language model to select the final answer. Our experiments show that our framework not only ensures monotonicity, but also outperforms state-of-the-art multi-source QA methods on Natural Questions. Additionally, we show that our models robustly preserve the monotonicity against noise from speech recognition. We publicly release our code and setting.

==> figures/previous_figures/figure_4_1.tex <==
\begin{figure}[t!]
%\centering
%         \includegraphics[width=1.0\linewidth]{figures/fig_method_spec_clean.pdf}
%    \hfill
     \centering
         \includegraphics[width=1.0\linewidth]{figures/fig_prelim_boxplot_v4.pdf}
\caption{Boxplot of the distributions of $P_{S}$ (left) and $P_{JS}$ (right) in NQ. The upper and lower edges of the box represent the upper quartile (highest 25\%) and the lower quartile (highest 75\%) values respectively. The median is represented as the line inside the box. }
\label{fig:figure_4_1}
\end{figure}

==> figures/previous_figures/figure_4_1_v1.tex <==
\begin{figure}[t!]
%\centering
%         \includegraphics[width=1.0\linewidth]{figures/fig_method_spec_clean.pdf}
%    \hfill
     \centering
         \includegraphics[width=1.0\linewidth]{figures/figure_boxplot_pspj.pdf}
\caption{Boxplot of the distributions of $P_{S}$ (left) and $P_{J}$ (right) in NQ. The upper and lower edges of the box represent the upper quartile (highest 25\%) and the lower quartile (highest 75\%) values respectively. The median is represented as the line inside the box. }
\label{fig:figure_4_1_v1}
\end{figure}

==> figures/previous_figures/figure_4_2.tex <==
\begin{figure}[t!]
     \centering
         \includegraphics[width=1.0\linewidth]{figures/fig_prelim_integ_v5_med.pdf}
         
\caption{Histogram of $P_{S}$ (left) and $P_{J}+P_{S}$ (right, scaled by 2) on NQ. Median value of each distribution is written in bold.}
\label{fig:figure_4_2}
\end{figure}

==> figures/previous_figures/figure_bs.tex <==
\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{0.36\textwidth}
         \includegraphics[width=\textwidth]{figures/bs_oracle.pdf}
         \caption{Correlation between oracle and beam size}
         \label{fig:bs_oracle}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.36\textwidth}
         \includegraphics[width=\textwidth]{figures/top1_beam.pdf}
         \caption{Selection by single reader}
         \label{fig:top1_beam}
     \end{subfigure}
\caption{In (a), as beam size increases, oracle also increases. In (b), the tendency that output in greedy search and top-1 output in beam search are little difference is observed. }
\label{fig:figure_bs}
\end{figure}

==> figures/previous_figures/figure_emt.tex <==
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.296\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_large.jpg}
         \caption{Judge debiasing (T5-large) }
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.296\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_base.jpg}
         \caption{Judge debiasing (T5-base)}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.338\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_pjs.jpg}
         \caption{Selection with different criteria}
     \end{subfigure}
    \caption{Discriminative calibration (TCD) and the performance (EM), observed with JS-vanilla in NQ.}
    \label{fig:figure_emt}
\end{figure*}

==> figures/previous_figures/figure_emt_copy.tex <==
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.296\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_large.jpg}
         \caption{Judge debiasing (T5-large) }
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.296\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_base.jpg}
         \caption{Judge debiasing (T5-base)}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.338\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/figure_emt_pjs.jpg}
         \caption{Selection with different criteria}
     \end{subfigure}
    \caption{Discriminative calibration (TCD) and the performance (EM), observed with JS-vanilla in NQ.}
    \label{fig:figure_emt}
\end{figure*}

==> figures/previous_figures/figure_oracle.tex <==
\begin{figure}[t!]
     \centering
         \includegraphics[width=0.9\linewidth]{figures/figure_oracle.jpg}
     \hfill
\caption{System recall (dotted line) and performance (bar) with regard to the beam budget in NQ.}
\label{fig:figure_oracle}
\end{figure}


==> figures/previous_figures/figure_ps_limitation.tex <==
\begin{figure}[t!]
     \centering
         \includegraphics[width=1.0\linewidth]{figures/figure_ps_limitation.jpg}
         
\caption{Accuracy of binary classification on NQ, by $P_{S}$ (bar) and $P_{J}$ (line).}
\label{fig:figure_ps_limitation}
\end{figure}

==> figures/previous_figures/figure_selected_probdist.tex <==
\begin{figure}[t!]
     \centering
         \includegraphics[width=0.9\linewidth]{figures/figure_selected_problist.jpg}
         
\caption{$P_{JS}$ distribution of selected candidates (left) and all candidates (right), represented with boxplot. Result from JS-vanilla in NQ.}
\label{fig:figure_selected_probdist}
\end{figure}

==> figures/previous_figures/figure_selection_ratio.tex <==
\begin{figure}[t!]
     \centering
         \includegraphics[width=1.0\linewidth]{figures/fig_selection_ratio_v1.pdf}
\caption{Selected percentage of each source, in candidate selection by $P_{S}$ and optimal selection. In optimal selection, [...]}
\label{fig:figure_selection_ratio}
\end{figure}

==> tables/RQ2.tex <==
\begin{table}
\centering
\begin{tabular}{lcc} 
\noalign{\hrule height 2pt} 
\multicolumn{1}{l}{\textbf{Method}} & T5-base & T5-large  \\ 
\hline
JS-vanilla (w/o JD)        & 49.5    & \textbf{55.4}      \\
JS-vanilla (w/ JD)         & \textbf{49.9}    & 55.2      \\
\hline
JS-lite (w/o JD)           & 49.3    & 53.5      \\
JS-lite (w/ JD)            & \textbf{49.6}    & \textbf{53.7}      \\
\noalign{\hrule height 2pt} 
\end{tabular}
\caption{Effect of judge debiasing, observed in NQ.}
\label{tab:RQ2}
\end{table}

%\textcolor{blue}{[ongoing]}

==> tables/ablation.tex <==
\begin{table}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l|cc}
\noalign{\hrule height 1pt} 
\multicolumn{1}{c}{\textbf{Method}}  & \textbf{EM}  \\ 
\noalign{\hrule height 1pt}
\textit{Individual Reader} & \\
~~ Text & 50.8 \\
~~ Table & 36.8 \\
~~ KB & 28.1 \\
%~~ Text + Table (*) & 53.7 \\
~~ Text + Table + KB  & 53.1  \\
% & ours                             &      &       \\ 
\hline
\textit{Selection in TT} & & \\
~~ $\text{P}_J + \text{P}_R$  & 55.4       \\
~~ $\text{P}_J$ only  & 55.2      \\
~~ $\text{P}_R$ only  & 49.9   \\
~~ Oracle  & 61.7   \\
\hline

\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Ablation study (greedy decoding)}
%We report the result of our `separate (Sep)' models where we use individual LMs for each knowledge source, together with `single' models where both documents and QA pairs are handled by one LM.}
\label{ablation}
\end{table}


%\begin{table}[t]
%\centering
%\scalebox{0.96}{
%\begin{tabular}{c|l|cc}
%\noalign{\hrule height 1pt} 
%Category & \multicolumn{1}{c|}{Knowledge Source}  & NQ   & TQA   \\ 
%\noalign{\hrule height 1pt}

%\multirow{5}{*}{Large} & Text   & 52.2   &  70.4   \\
%& Table    & 55.1 &  71.7    \\ 
%& KB    & 54.9  & 72.4  \\
%& Text + Table    & 54.9  & 72.4  \\ 
%& Text + Table + KB    & 54.9  & 72.4  \\ 
%\hline
%\multirow{5}{*}{Xlarge} & Ours: (1) LM prob   & 54.5  & 73.5      \\
% & Ours: (1) LM prob    & 56.3 &      \\ 
%& Ours: (2) Answerability  & 57.6 & 74.2     \\ 
%& Ours: (3) Consistency    & 57.0 & 74.3     \\  
%& Ours: (1+2+3)    & \textbf{58.1} & \textbf{74.7}     \\  
%& Oracle - Upper Bound  & 64.6 & 77.5    \\
%\noalign{\hrule height 1pt} 
%\end{tabular}}
%\caption{Ablation Study}
%\label{ablation}
%\end{table}

==> tables/analysis_cp.tex <==
\begin{table}
\centering
\begin{tabular}{lcc} 
\noalign{\hrule height 2pt} 
\textbf{Policy}             & \textbf{Avg beam size} & \textbf{EM}    \\ 
\hline
no policy          & 5             & 56.0  \\
static policy      & 3             & \textbf{56.3} \\
\noalign{\hrule height 2pt} 
\end{tabular}
\caption{Average beam size and EM in no policy and static policy.}
\label{tab:analysis_cp}
\end{table}


==> tables/analysis_distill.tex <==

\begin{table}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l|cc}
\noalign{\hrule height 1pt} 
\multicolumn{1}{c}{Method}  & NQ & WQ (*) \\ 
\noalign{\hrule height 1pt}
~~ Text & 47.5 & 23.8 \\
~~ Table & 31.6 & 19.0 \\
~~ KB  & 15.7 & 13.6  \\
~~ Selection ($\text{P}_R$)  & \textbf{51.1} & \textbf{25.1} \\

\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Distillation result. WQ(*) is OOD.}

\label{distill_result}
\end{table}

==> tables/analysis_judge.tex <==
\begin{table}[t]
\centering
\scalebox{0.96}{
\begin{tabular}{c|l|cc}
\noalign{\hrule height 1pt} 
Judge & \multicolumn{1}{c|}{Knowledge source}  & EM   \\ 
\noalign{\hrule height 1pt}

\multirow{4}{*}{TT reader} & Text + Table   & 55.2   \\
& Text + Table + KB    & 55.4    \\
& Text + Table (bs)   & 56.2   \\
& Text + Table + KB (bs)    & 56.6    \\
\hline
\multirow{4}{*}{TTK reader} & Text + Table   & 54.9   \\
& Text + Table + KB    & 55.0    \\
& Text + Table (bs)   & 56.0   \\
& Text + Table + KB (bs)    & 56.3    \\
\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Selection EM in NQ.}
\label{judge_performance}
\end{table}

==> tables/analysis_moe.tex <==
\begin{table}
\centering
\begin{tabular}{lccc} 
\noalign{\hrule height 1pt} 

\textbf{Method}  &  \textbf{Text} & \textbf{TT}   & \textbf{TTK}   \\ 
\hline
MTL-1 & 41.8 & 45.7 & 46.1  \\
MTL-2 (ours) & 45.1 & 49.3 & 49.5  \\
\noalign{\hrule height 1pt} 
\end{tabular}
\caption{Comparison of results of MoE and our version of MTL in NQ. Models are implemented on T5-base.}
\label{tab:analysis_moe}
\end{table}



==> tables/analysis_selection.tex <==


\begin{table}[]
\centering
\begin{tabular}{|cc|cc|}
\hline
\multicolumn{2}{|c|}{}                                                                                        & \multicolumn{2}{c|}{\textbf{Selection in TTK}}         \\ 
\cline{3-4} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}KB reader \\ True\end{tabular}}}} & \multicolumn{1}{c|}{\textit{True}}                      & \textit{False} \\ 
\hline
\multicolumn{1}{|c|}{}                                                         & \textit{True}                         & \multicolumn{1}{c|}{848}                       & 31    \\ 
\cline{2-4} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}} Unify \\ (TTK) \end{tabular}}}}                        & \textit{False}                        & \multicolumn{1}{c|}{{\textbf{99}}} & 38    \\ 
\hline
\end{tabular}
\caption{Results of NQ test indicating how much unified-based model and selection-based model (ours) were correct in the data that KB reader was correct, respectively.}
\label{tab:selection_result}
\end{table}

==> tables/analysis_webq_selection.tex <==


\begin{table}[]
\centering
\begin{tabular}{|cc|cc|}
\hline
\multicolumn{2}{|c|}{}                                                                                        & \multicolumn{2}{c|}{\textbf{Selection in TT}}         \\ 
\cline{3-4} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Table reader \\ True\end{tabular}}}} & \multicolumn{1}{c|}{\textit{True}}                      & \textit{False} \\ 
\hline
\multicolumn{1}{|c|}{}                                                         & \textit{True}                         & \multicolumn{1}{c|}{289}                       & 13    \\ 
\cline{2-4} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}} Unify \\ (TT) \end{tabular}}}}                        & \textit{False}                        & \multicolumn{1}{c|}{{\textbf{64}}} & 85    \\ 
\hline
\end{tabular}
\caption{Results of WQ(*) test indicating how much unified-based model and selection-based model (ours) were correct in the data that Table reader was correct, respectively.}
\label{tab:webq_selection}
\end{table}


==> tables/answerable_em.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\noalign{\hrule height 1pt}
{\textbf{Source}}                    & {\textbf{R@50}}   & {\textbf{Total EM}}  & {\textbf{Oracle-Ret EM}} \\ 
\hline
\multicolumn{1}{c}{{Text}} & {84.9} & {50.9} & {\textbf{58.7}    \\
\multicolumn{1}{c}{{TT}}   & {90.3} & {53.7} & {\textbf{58.9}}    \\
\multicolumn{1}{c}{{TTK}}  & {89.1} & {53.1} & {\textbf{59.0}}    \\ \hline
\noalign{\hrule height 1pt}
\end{tabular}
\caption{The performance of unified retrievers and readers in NQ.}
%SE - alternative to Oracle?
\label{answerable_em}
\end{table}
\begin{comment}
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\noalign{\hrule height 1pt}
{\textbf{Source}}                    & {\textbf{R@50}}   & {\textbf{Total EM}}  & {\textbf{Oracle-Ret EM}} \\ 
\hline
\multicolumn{1}{c}{{Text}} & {84.90} & {50.89} & {\textbf{58.69}}    \\
\multicolumn{1}{c}{{TT}}   & {90.33} & {53.74} & {\textbf{58.91}}    \\
\multicolumn{1}{c}{{TTK}}  & {89.11} & {53.07} & {\textbf{58.97}}    \\ \hline
\noalign{\hrule height 1pt}
\end{tabular}
\caption{The performance of unified retrievers and readers in NQ.}
%SE - alternative to Oracle?
\label{answerable_em}
\end{table}
\end{comment}

==> tables/webq_result.tex <==
\begin{table}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l|cc}
\noalign{\hrule height 1pt} 
\multicolumn{1}{c}{\textbf{Method}}  & \textbf{EM}  \\ 
\noalign{\hrule height 1pt}
\textit{Individual Reader} & \\
~~ Text & 26.0 \\
~~ Table & 22.2 \\
~~ Text + Table & 25.2 \\
% & ours                             &      &       \\ 
\hline
\textit{Selection in TT} & & \\
~~ $\text{P}_R$ only  & 27.4   \\
~~ $\text{P}_J$ only  & 28.1      \\
~~ $\text{P}_J + \text{P}_R$  & 28.0       \\
\hline

\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Results of WQ(*). The model trained in NQ was applied to WQ(*), which is OOD.}
\label{tab:webq_result}
\end{table}


\begin{comment} % previous version
\begin{table}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l|cc}
\noalign{\hrule height 1pt} 
\multicolumn{1}{c}{\textbf{Method}}  & \textbf{EM}  \\ 
\noalign{\hrule height 1pt}
\textit{Individual Reader} & \\
~~ Text & 26.0 \\
~~ Table & 22.2 \\
~~ KB & 21.3 \\
~~ Text + Table & 25.2 \\
~~ Text + Table + KB  & 24.8  \\
% & ours                             &      &       \\ 
\hline
\textit{Selection in TT} & & \\
~~ $\text{P}_R$ only  & 27.4   \\
~~ $\text{P}_J$ only  & 28.1      \\
~~ $\text{P}_J + \text{P}_R$  & 28.0       \\
\hline
\textit{Selection in TTK} & & \\
~~ $\text{P}_R$ only  & 28.2   \\
~~ $\text{P}_J$ only  & 28.4      \\
~~ $\text{P}_J + \text{P}_R$  & 28.5       \\
\hline

\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Results of WQ(*). The model trained in NQ was applied to WQ(*), which is OOD.}
\label{tab:webq_result}
\end{table}
\end{comment}
